ASR-Aware End-to-end Neural Diarization

We present a Conformer-based end-to-end neural diarization (EEND) model that uses both acoustic input and features derived from an automatic speech recognition (ASR) model. Two categories of features are explored: features derived directly from ASR output (phones, position-in-word and word boundaries) and features derived from a lexical speaker change detection model, trained by fine-tuning a pretrained BERT model on the ASR output. Three modifications to the Conformer-based EEND architecture are proposed to incorporate the features. First, ASR features are concatenated with acoustic features. Second, we propose a new attention mechanism called contextualized self-attention that utilizes ASR features to build robust speaker representations. Finally, multi-task learning is used to train the model to minimize classification loss for the ASR features along with diarization loss. Experiments on the two-speaker English conversations of Switchboard+SRE data sets show that multi-task learning with position-in-word information is the most effective way of utilizing ASR features, reducing the diarization error rate (DER) by 20% relative to the baseline.

==> data_table2.tex <==
\begin{table}[h]
\begin{center}
%\small
\caption{Multi-task (MT) training combined with speaker change (SC) prediction features. Baseline DER with LFBE only is 3.19\%. Relative improvement \% in brackets.}
\vspace{-2mm}
\label{table:results2}
\begin{tabular}{c c c | c}
\toprule
MT features & SC features & SC config & DER (\%) \\
 \midrule
 -  & Posteriors & Late fusion                & 2.88 (9.72\%) \\
Word position  & - & -                        & 2.54 (20.38\%) \\
Word position  & Posteriors &  Late fusion    & 2.61 (18.18\%)\\
\bottomrule
\end{tabular}
\end{center}
\vspace{-2mm}
\end{table}

